Causal Abstraction with Soft Interventions

Causal abstraction provides a theory describing how several causal models can represent the same system at different levels of detail. Existing theoretical proposals limit the analysis of abstract models to "hard" interventions fixing causal variables to be constant values. In this work, we extend causal abstraction to "soft" interventions, which assign possibly non-constant functions to variables without adding new causal connections. Specifically, (i) we generalize $\tau$-abstraction from Beckers and Halpern (2019) to soft interventions, (ii) we propose a further definition of soft abstraction to ensure a unique map $\omega$ between soft interventions, and (iii) we prove that our constructive definition of soft abstraction guarantees the intervention map $\omega$ has a specific and necessary explicit form.

==> figures/explicitomega.tex <==
\definecolor{qcolor}{RGB}{127, 161, 170}
\definecolor{pcolor}{RGB}{222, 181, 106}
\definecolor{icolor}{RGB}{180, 40, 40}
\definecolor{ycolor}{RGB}{74, 154, 71}

\begin{figure}
\centering
\begin{tikzpicture}[minimum width=0.5cm]
{
  % Higher Level Before
  \node[draw, circle,fill=pcolor] (P) at (-5, -2) {$P$};
  \node[draw, circle,fill=qcolor] (Q) at (-5, -4) {$Q$};
  \node[draw, circle] (H) at (-4, -3) {$Y$};
  \draw[-{Latex}] (P)--(Q);
  \draw[-{Latex}] (P)--(H);
  \draw[-{Latex}] (Q)--(H);
  % Box
  \node[draw=none,rectangle,fit=(P) (Q) (H)] (PQH) {};

  % Lower Level
  % \Pi(p)
  \node[draw, circle,fill=pcolor] (LP1) at (0, 0) {};
  \node[draw, circle,fill=pcolor] (LP2) at (-1, -1) {};
  \node[draw, circle,fill=pcolor] (LP3) at (1, -2) {};
  \node[draw=none,rectangle,fit=(LP1) (LP2) (LP3),label={left:$\Pi(P)$}] (LP) {};
  % \Pi(q)
  \node[draw, circle,fill=qcolor] (LQ1) at (-1, -3) {};
  \node[draw, circle,fill=qcolor] (LQ2) at (1, -4) {};
  \node[draw, circle,fill=qcolor] (LQ3) at (0, -5) {};
  \node[draw=none,rectangle,fit=(LQ1) (LQ2) (LQ3),label={[yshift=-1cm,xshift=0.1cm]left:$\Pi(Q)$}] (LQ) {};
  % \Pi(h)
  \node[draw, circle,fill=ycolor] (LH1) at (3, -3) {};
  \node[draw, circle,fill=ycolor] (LH2) at (4, -2) {};
  \node[draw, circle,fill=ycolor] (LH3) at (4, -4) {};
  \node[draw, circle,fill=ycolor] (LH4) at (5, -3) {};
  \node[draw=none,rectangle,fit=(LH1) (LH2) (LH3) (LH4),label={$\Pi(Y)$}] (LH) {};
  % External
  % \node[draw, circle,label={left:$X_c$}] (EXT) at (3, -5) {};
  % Connections
  \draw[-{Latex}] (LP2)--(LP1);
  \draw[-{Latex}] (LP2)--(LP3);
  \draw[-{Latex},color=icolor,densely dotted] (LP1)--(LH2);
  \draw[-{Latex}] (LP3)--(LH1);
  \draw[-{Latex}] (LP2)--(LQ1);
  \draw[-{Latex}] (LQ1)--(LQ2);
  \draw[-{Latex}] (LQ1)--(LQ3);
  \draw[-{Latex}] (LQ2)--(LH1);
  \draw[-{Latex}] (LQ3)--(LQ2);
  \draw[-{Latex}] (LQ3)--(LH3);
  % \draw[-{Latex}] (EXT)--(LH3);
  \draw[-{Latex},color=icolor] (LH1)--(LH2);
  \draw[-{Latex}] (LH1)--(LH3);
  %\draw[-{Latex},color=icolor,densely dotted] (LH1)--(LH4);
  \draw[-{Latex}] (LH1)--(LH4);
  \draw[-{Latex}] (LH3)--(LH4);
  % Box
  % \node[draw=none,rectangle,fit=(LP) (LQ) (LH) (EXT)] (LOWER) {};
  \node[draw=none,rectangle,fit=(LP) (LQ) (LH)] (LOWER) {};

  % Higher After
  \node[draw, circle] (P2) at (8, -2) {$P$};
  \node[draw, circle] (Q2) at (8, -4) {$Q$};
  \node[draw, circle,fill=ycolor] (H2) at (9, -3) {$Y$};
  \draw[-{Latex}] (P2)--(Q2);
  \draw[-{Latex}] (P2)--(H2);
  \draw[-{Latex}] (Q2)--(H2);
  % box
  \node[draw=none,rectangle,fit=(P2) (Q2) (H2)] (PQH2) {};

  % Connect boxes
  \draw[-{Latex},dotted,thick] (-3.2, -3)--(-1.5, -3);
  \draw[-{Latex},dotted,thick] (5.5, -3)--(7.5, -3);
  \draw[-{Latex},dotted,thick] (1, 0)--(3, 0);
  
  % Strike through arrow
  % \node[draw=none](STRIKE) at ($(LH1)!0.5!(LH4)$){\color{icolor}\Large\textbf{/}};
  \node[draw=none](STRIKE) at ($(LP1)!0.5!(LH2)$){\color{icolor}\Large\textbf{/}};
  
  \node[draw=none, yshift=0.4cm](BACK) at ($(-3.2, -3)!0.5!(-1.5, -3)$){\large$\tau^{-1}_{\pa(Y)}$};
  \node[draw=none, yshift=0.3cm](FORWARD) at ($(5.5, -3)!0.5!(7.5, -3)$){\large$\tau_{Y}$};
  \node[draw=none, yshift=0.3cm](TWO) at ($(1, 0)!0.5!(3, 0)$){\large$F^{\color{icolor}i}_{\Pi(Y)}$};
}
\end{tikzpicture}
\caption{
Given an intervention {\color{icolor}$i$} on a set of lower-level variables abstracted by the higher-level variable {\color{ycolor}$Y$}, we prove that the corresponding high-level intervention has form $Y \gets g$.
Furthermore, we show that the resulting function $g$ depends at most on parents $\pa(Y)$ and consists of the composition of three functions: the inverse mapping $\tau^{-1}$, the intervened structural equations $F^{\color{icolor}i}$, and the mapping $\tau$.
Notably, even if $\tau_{\pa(Y)}$ is not invertible, the composition is defined for any function mapping to the original high-level values.
}\label{fig:explicitomega}
\end{figure}
